Deep-Edge: An Efficient Framework for Deep Learning Model Update on Heterogeneous Edge

Deep Learning (DL) model-based AI services are increasingly offered in a variety of predictive analytics services such as computer vision, natural language processing, speech recognition. However, the quality of the DL models can degrade over time due to changes in the input data distribution, thereby requiring periodic model updates. Although cloud data-centers can meet the computational requirements of the resource-intensive and time-consuming model update task, transferring data from the edge devices to the cloud incurs a significant cost in terms of network bandwidth and are prone to data privacy issues. With the advent of GPU-enabled edge devices, the DL model update can be performed at the edge in a distributed manner using multiple connected edge devices. However, efficiently utilizing the edge resources for the model update is a hard problem due to the heterogeneity among the edge devices and the resource interference caused by the co-location of the DL model update task with latency-critical tasks running in the background. To overcome these challenges, we present Deep-Edge, a load- and interference-aware, fault-tolerant resource management framework for performing model update at the edge that uses distributed training. This paper makes the following contributions. First, it provides a unified framework for monitoring, profiling, and deploying the DL model update tasks on heterogeneous edge devices. Second, it presents a scheduler that reduces the total re-training time by appropriately selecting the edge devices and distributing data among them such that no latency-critical applications experience deadline violations. Finally, we present empirical results to validate the efficacy of the framework using a real-world DL model update case-study based on the Caltech dataset and an edge AI cluster testbed.

==> Motivation.tex <==
\section{Motivation}
\label{sec:motivation}
This section focuses on the motivation behind developing the DeepEdge framework. Here, we describe how a DL model degrades in the presence of new data, and why we should update the existing DL model. We describe the motivation behind distributed training and the impact of resource interference on DL model training time under various stressed conditions.

\subsection{Motivation for Model Update}
We use an example of mapping images to steering angle control in the autonomous car with CARLA \cite{dosovitskiy2017carla}, an autonomous driving simulator, to explain how the model degrades when the initially trained images are synthetically changed with rain ntensities~\cite{tian2018deeptest}. In our experiments, we used the inbuilt controller to drive the car on a bright sunny day, and collect 5000 front dashboard camera images at five fps (frames per second) along with the steering data for training a neural network model. Using the labeled data, we trained an NVIDIA's DAVE-II CNN model \cite{bojarski2016end} to learn the steering actions. We trained the model for 50 epochs and evaluated its performance on a validation dataset, for which we got a mean square error (MSE) of 0.0078 (lower is better). For evaluating the models' performance for different weather conditions, we chose a single straight road seen during training and then deployed the trained model to perform the steering actions. Figure \ref{Fig:dist0} shows the absolute error between the actual steering and the model steering predictions for the entire experimental evaluation. For the first 150 simulation steps, we maintain sunny weather, so the absolute error is minimal, and in the next simulation step, we change to rainy weather. With the new rainy condition, the error increases, and here we collect the images for 100 simulation steps with corrected steering value\footnotetext[2]{We assume that there will be a human-in-the-loop who will correct the steering angle if the DL model predicts wrong. } and then triggered the model update. It takes about 10 seconds (50 simulation steps) to get the model updated. At step 301, we deploy the updated model, and we see the error goes low compared to the error before it was retrained.  Figure \ref{Fig:dist0} also illustrates that the error continues to be high if the model is not updated.

\begin{figure}[tbh]
	\centering
	\includegraphics[width=0.9\linewidth]{images/dist_motivation0.pdf}\vskip -1mm
	\caption{ Absolute error between predicted steering value and the actual steering value (with and without model update) }
	\label{Fig:dist0}
	\vskip -2mm
\end{figure}

Similar model degradation was also observed for the DL-based image classifiers when we emulate the training on a small chunk of data from the Caltech dataset~\cite{fei2004learning}. As we change the test dataset to new data, the model degrades over time, and the experiment motivates the need for an online DL model updating with unseen images to make the model robust. 

\subsection{Motivation for Distributed Training}
Our application is based on DL model training on Caltech dataset~\cite{fei2004learning} using MxNet framework~\cite{chen2015mxnet}. We trained our model on 3855 data points with different resource configurations and batch size. 

We did our experiments on Jetson Nano devices on standalone mode and in distributed (asynchronous-centralized) mode. For the first experiment, we ran the experiment in standalone mode with 8 and 16 batch size. As shown in Figure~\ref{Fig:dist}, increasing batch size reduces the per epoch training time, because of less number of updates. For the second set of experiments, we distributed the training data equally (1928 and 1927 data points respectively) on 2 Jetson Nano worker nodes and used the Jetson TX2 device as the parameter server.  We changed the batch size among  8, and 16 in all worker nodes, respectively\footnotetext[1]{We considered maximum batch size as 16, because Nano is limited to 4GB memory, and bigger batch size than 16 for CalTech DL model exceeds the memory of Nano device. The batch size limit for the TX2 device(8GB memory) is 64. }. As shown in Figure~\ref{Fig:dist}, training time reduced when we distributed training over a single Jetson Nano device. For the third set of experiments, we distributed the training data equally (1285 points on each node) on 3 Jetson Nano worker nodes and used the Jetson TX2 device as a parameter server. Similarly, we observed significant improvement in training time by distributing the data points on three worker nodes over a single Jetson Nano device; however, the training time suffers significantly because of communication overhead. Therefore, we should consider the communication impact on distributing DL training in multiple machines~\cite{chen2015mxnet}.

\begin{figure}[tbh]
	
	\centering
	\begin{subfigure}[t]{0.24\textwidth}
		\centering
		\includegraphics[width = \linewidth]{images/dist_motivation.pdf}\vskip -1mm
		\caption{\scriptsize DL model training time (per epoch) for different resource configurations and different batch sizes.}
		\label{Fig:dist}
	\end{subfigure}%
	~
	\centering
	\begin{subfigure}[t]{0.24\textwidth}
		\centering
		\includegraphics[width = \linewidth]{images/dist_motivation1.pdf}\vskip -1mm
		\caption{\scriptsize DL model training time (per epoch) on standAlone TX2 and on heterogeneous cluster with different batch sizes.}
		\label{Fig:dist1}
	\end{subfigure}%
	\caption{Per Epoch Training time with different configurations }\vskip -5mm
	\label{Fig:dist_fig}
	\vskip 2mm
\end{figure}

\textbf{\textit{Impact of Heterogeneity.}} 
In this experiment, we trained our model on 3855 data points on a single Jetson TX2 device. Then, we distributed the training data equally (1285 points on each node) among 2 Jetson Nano worker nodes and a Jetson TX2 device. We used another Jetson Nano device as a parameter server. We conducted experiments with maximum possible batch size combinations on each device. Figure \ref{Fig:dist1} illustrates that distributed training in these experiments was less efficient than doing the same training on the most powerful device, i.e., Jetson TX2. Moreover, because of the same amount of data points among all the worker nodes, TX2 was idle for a significant amount of time. Hence, finding the proper ratio of data and map that among the heterogeneous devices is challenging, and this motivates our study to find the near-optimal data ratio to minimize the overall job completion time.

Furthermore, the edge devices may process a background task. Hence, their available resources limit the selection of batch size, available CPU, GPU, and IO, which may impact the total job completion time. Moreover, changing the number of worker nodes and the ratio of data mapping to the resources might also impact the total training time.
We only considered the production DL models, which converge to the desired accuracy eventually.  


\subsection{Motivation to Study Resource Interference}
We trained our DL model on 2570 data points with batch size 16 on the NVIDIA Jetson TX2 device, and measured the time to process each batch in isolation, and co-located with background CPU-intensive and CPU-IO-intensive applications.

\begin{figure}[tbh]
	\centering
	\includegraphics[width=0.9\linewidth]{images/resourceInterferenceGraph.pdf}\vskip -1mm
	\caption{  CDF representation of training times per batch in isolation, and co-located with background CPU-intensive and CPU-IO-intensive applications. }
	\label{Fig:interference}
	\vskip -2mm
\end{figure} 

Application performance degrades when co-located with resource-intensive background applications because of resource interference. Figure \ref{Fig:interference} illustrates that the application’s performance degrades 5\% and 11\% when co-located with background CPU-intensive and CPU-IO-intensive applications, respectively,  as compared to its performance when running in isolation. This motivates us to study the resource-interference thoroughly to understand the impact of resource interference on training time.

==> casestudies.tex <==
\section{Evaluation}
\label{sec:casestudies}

We evaluated our implementation of the DeepEdge framework and proposed heuristic with multiple DNN models on heterogeneous edge clusters.

\subsection{Experiment Setup}
\subsubsection{Testbed} 
We conducted all our experiments on the edge cluster comprised of one \emph{NVIDIA Jetson TX2} (256-core NVIDIA Pascal GPU, 8GB memory, Dual-Core NVIDIA Denver 2 64-Bit CPU and Quad-Core ARM Cortex-A57), three \emph{NVIDIA Jetson Nano} ( 128-core Maxwell GPU, Quad-Core ARM Cortex-A57, 4GB memory) devices and one \emph{Raspberry Pi 4} (Broadcom BCM2711, Quad-core Cortex-A72 (ARM v8), 4GB memory) devices, and connected by one Gigabit switch. We considered the Raspberry Pi device as our \emph{parameter server} for all the experiments of distributed deep-learning.

\subsubsection{Workloads} 
Our application is based on a prototype of image classification deep learning model, which is built using transfer learning~\cite{yosinski2014transferable} on the pre-trained ResNet and Inception models on Caltech dataset~\cite{fei2004learning} using MxNet framework~\cite{chen2015mxnet}. 

\subsubsection{Methodology} 
We built our base model using transfer learning and trained it using 2570 data points of the Caltech dataset. The base model achieved 75\% accuracy on our validation dataset. We emulated the model update trigger when the accuracy of the base model decreases below 50\% accuracy, which is our assumed tolerance threshold. To emulate real data generation, we continuously feed the base model new 4600 data points, where the model accuracy degraded to 50\% accuracy, and we triggered the model update process. We updated our model on 4600 data points of the Caltech dataset, in which 3855 data points are used as training data points, and the rest of the data points are validation set. 

\subsection{Sensitivity Analysis of the DL Model Update}
As described in Section~\ref{sec:perf_model}, we have to identify the feature sets of the background applications, which affects the performance of the \textit{epochTime} of the DL model update job. \textit{epochTime} is the summation of \textit{t$_{compute}$} and \textit{t$_{update}$}, so we studied the effect of background jobs on t$_{compute}$ and t$_{update}$ separately. To emulate the behavior of background jobs, we develop the stressors to stress the nodes along multiple dimensions (GPU, CPU, memory, and IO). We also did multiple experiments while changing the batch size of the DL model update task. Recall, memory limits the batch size of the DL model update task.

Based on our sensitivity analysis, we observed the behaviors as follows:
\Romannum{1}. Stressing GPU increase compute time($t_{compute}$)  as shown in Figure~\ref{Fig:GPU_Time}.
\begin{figure}[tbh]
	\centering
	\includegraphics[width = 0.8\linewidth]{images/GPU_Time.pdf}\vskip -1mm
	\caption{\scriptsize Stressing GPU increases compute time.}
	\label{Fig:GPU_Time}
\end{figure}
\Romannum{2}. Stressing CPU and IO increase compute time.
\begin{figure}[tbh]
	\centering
	\includegraphics[width = 0.8\linewidth]{images/batch_Mem.pdf}
	\caption{\scriptsize Increasing the batch size increases the memory footprint.}
	\label{Fig:batch_Mem}
\end{figure}
\Romannum{3}.  Increasing the batch size of the DL model update process increases the memory footprint as shown in Figure~\ref{Fig:batch_Mem}, but increasing batch size decreases compute time($t_{compute}$) as shown in Figure~\ref{Fig:batch_compute}.
\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{images/batch_compute.pdf}
	\caption{Increasing Batch size decreases compute time.}
	\label{Fig:batch_compute}
\end{figure}
\Romannum{4}.  Increase the number of workers results in the DL model update time($t_{update}$) increase as shown in Figure~\ref{Fig:worker_update}.
\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{images/worker_update.pdf}
	\caption{Increasing workers nodes increase update time.}
	\label{Fig:worker_update}
\end{figure}
\Romannum{5}.  Stressing CPU of parameter server, which is Raspberry Pi for our experiments, increases update time($t_{update}$) as shown  in Figure~\ref{Fig:ps_update}.
\begin{figure}[tbh]
	\centering
	\includegraphics[width=0.8\linewidth]{images/ps_update.pdf}
	\caption{Stressing CPU of parameter server increases update time.}
	\label{Fig:ps_update}
\end{figure}
\Romannum{6}.  Memory, IO of parameter server do not affect the update time.
\Romannum{7}.  Decreasing the batch size also increases the update time.
This sensitivity analysis shows how the DL model update time can vary based on the state of the nodes($\mathcal{X}_i$).


\subsection{Pressure of model update on background jobs}
As described in Section~\ref{sec:perf_model}, we also have to estimate the pressure of the DL model update job on the background latency-critical jobs. If the estimated pressure of the DL model update jobs goes beyond a threshold limit($\delta^a$), which is pre-defined by the background applications, we do not consider the node for the DL model update task. We have studied the behavior of the DL model tasks by changing the initial state of the nodes, and figure out how much pressure the DL model update task exerts in multiple dimensions (GPU, CPU, memory, and IO). we observed the behaviors as follows:
\Romannum{1}. Running DL model update task increases the CPU usage of the worker node as shown in Figure~\ref{Fig:Initital_Final_CPU}.
\begin{figure}[tbh]
	\centering
	\includegraphics[width = 0.8\linewidth]{images/Initital_Final_CPU.pdf}
	\caption{\scriptsize Initial and Final CPU Usage.}
	\label{Fig:Initital_Final_CPU}
\end{figure}
\Romannum{2}. Running DL model update task saturates the GPU of the worker node as shown in Figure~\ref{Fig:Initital_Final_GPU}.
\begin{figure}[tbh]
	\centering
	\includegraphics[width = 0.8\linewidth]{images/Initital_Final_GPU.pdf}
	\caption{\scriptsize Initial and Final GPU Usage.}
	\label{Fig:Initital_Final_GPU}
\end{figure}
\Romannum{3}. Running DL model update task increases the memory footprint of the worker nodes.

\subsection{Effectiveness of Data Sharding Strategy}
As described in Section~\ref{sec:perf_estimation}, we develop a heuristic to shard the data among the worker nodes so that that the epoch time in all the workers remains the same. Recall, epoch time is $B_i (b_i \cdot t_i^{compute} + t_i^{update})$, where $B_i$ is the number of batches, and $b_i$ is batch size of the worker$_i$.
\begin{figure}
	\centering
	\includegraphics[width= 0.9\linewidth]{images/experiment_1.pdf}
	\caption{Epoch time with different cluster setup.}
	\label{Fig:experiment_1}
\end{figure}

As described in Algorithm~\ref{algo:shardinglogic}, we calculated the number of data points for each worker from the whole dataset, and send the respective data points($d_i$) to respective workers. In isolation, TX2 devices support the batch size of 64 for the Caltech dataset, whereas Nano devices support the batch size of 16 for the Caltech dataset. This is because, TX2 device has 8GB memory, where the Nano device has 4GB memory space. We considered the maximum available batch size, because increasing batch size results decrease in the compute and update time. For our experiments, we had one TX2 and three Nano devices. Based on our performance estimation algorithm, we divided 1893 data points for the one TX2 device and 654 data points for the three Nano devices. The epoch time for the experiment in the heterogeneous cluster was around 121 seconds, as shown in the Figure~\ref{Fig:experiment_1}(a). After that, our Algorithm~\ref{algo:shardinglogic} removes the slowest worker node and calculates the epoch time. Here, as shown in Figure~\ref{Fig:experiment_1}(b), removing one worker increases the epoch time, and it becomes around 148 seconds. Then, we compared the epoch time with the best performing standalone device. In this case, if we run the experiment on a standalone TX2 device with 3855 data points, the epoch time would be around 184 seconds. Therefore, based on these experiments, we considered one TX2 and three Nano devices cluster setup for the model update task because, in that setup, the epoch time was minimum, as shown in Figure~\ref{Fig:experiment_1}.

\begin{figure}[tbh]
\begin{subfigure}{0.5\columnwidth}
	\centering
	\includegraphics[width=\linewidth]{images/GPUState1.pdf}		\vskip -2mm
	\caption{}
\end{subfigure}%%
~
\begin{subfigure}{0.5\columnwidth}
	\centering
	\includegraphics[width=\linewidth]{images/GPUState2.pdf} \vskip -2mm
	\captionsetup{width=0.8\linewidth}
	\caption{}
\end{subfigure}
\caption{EpochTime when GPU is occupied by co-located application}
\label{Fig:GPUsate}
\end{figure}

In our second case study, we ran GPU intensive tasks as background co-located applications. In this experiment, the GPU utilization in TX2 was 32$\%$ due to background co-located applications. In the first Nano device GPU utilization was 42$\%$, and in the other two Nano devices the GPU utilization was 24$\%$ due to background co-located applications. 
With this background GPU utilization, we run the DL model update task in the heterogeneous cluster. Using the  Algorithm~\ref{algo:shardinglogic}, we calculate the number of data points for each worker, so that the epoch time remains the same. Based on our performance estimation algorithm, we divided 1631 data points for the one TX2 device, 691 data points for the first Nano device, 769 data points for the second Nano device, and 764 datapoints for third Nano device. As shown in the Figure~\ref{Fig:GPUsate}(a), the epoch time for all the devices is around 154 seconds in the four worker node cluster setup.

Similarly, we changed the background co-located tasks to change the background GPU utilizations. The GPU utilization in TX2 was 28$\%$ due to background co-located applications. In the first Nano device GPU utilization was 25$\%$, and in the other two Nano devices the GPU utilization was 24$\%$ due to background co-located applications. Based on our performance estimation algorithm, we divided 1677 data points for the one TX2 device, 694 data points for the first Nano device, 735 data points for the second Nano device, and 749 datapoints for third Nano device. As shown in the Figure~\ref{Fig:GPUsate}(b), the epoch time for all the devices is around 155 seconds in the four worker node cluster setup. 

\subsection{Model Convergence}
As shown in the Figure~\ref{Fig:Model_conv}, the model always converges despite of different batch combinations and different computing power of the edge devices.\\
\todo{Will explain}
\begin{figure}[tbh]
	\begin{subfigure}{0.9\columnwidth}
		\centering
		\includegraphics[width=\linewidth]{images/Model_conv1.pdf}		\vskip -2mm
		\caption{\scriptsize With batch combination of 64,16,16,16 on  cluster of 1tx2 and 3 nanos
		}
	\end{subfigure}%%
	
	\begin{subfigure}{0.9\columnwidth}
		\centering
		\includegraphics[width=\linewidth]{images/Model_conv2.pdf} \vskip -2mm
		\captionsetup{width=\linewidth}
		\caption{\scriptsize With batch combination of 8,8,8,8 on  cluster of 1tx2 and 3 nanos
		}
	\end{subfigure}
	\caption{Model convergence in the distributed DL training}
	\label{Fig:Model_conv}
\end{figure}

==> future.tex <==
% $Id$
By surveying the literature in Section~\ref{sec:survey}, we find
some gap needs to filled for automatic transformation of the
business-relevant model to TOSCA-compliant deployable model. First, we
need to define a metamodel for the business user, who makes the model
on top of that without the need to be a domain expert.  The metamodel
will then transform the user model to TOSCA-compliant deployable model
in an efficient and optimal way and will also guarantee the
correctness of the model. The Aeolus project approach is a good
solution to reach the goal, but it did not build on top of TOSCA
specification which is a standard.  On the other hand, OpenTOSCA
approach is TOSCA-compliant, but it lacks the robustness of the CSP
solver. 

We built the metamodel for the business user using a web version of
GME (Generic Modeling Environment)
toolkit~\cite{ledeczi2001generic}. It is a toolkit for creating a
Domain Specific Modeling Language (DSML) through metamodel specifying
the modeling language of the application domain. In the modeling
language, we specified all the syntactic, semantic, and presentation
information regarding the domain, which needs to be used to construct
deployable models using ansible.  We created the model for this
transformation in webGME, which will be the metamodel for the
users. We provided specific interpreters for our WebGME model, which
convert any user-defined model to a TOSCA-compliant Ansible deployable
model.   

In future, our DSML generated ansible script needs to be verified
using a CSP solver, and it will prove its soundness and robustness. We
would also like to add type-based and AI-based pattern matching
approach for finding software dependencies, and we can make our DSML
learn from the history by using machine-learning techniques.  The
migration of application components is also a necessary feature
which needs to be automated. 

